Absorb & Escape: Overcoming Single Model Limitations in Generating Genomic Sequences

Abstract Recent advances in immunology and synthetic biology have accelerated the development of deep generative methods for DNA sequence design. Two dominant approaches in this field are AutoRegressive (AR) models and Diffusion Models (DMs). However, genomic sequences are functionally heterogeneous, consisting of multiple connected regions (e.g., Promoter Regions, Exons, and Introns) where elements within each region come from the same probability distribution, but the overall sequence is non-homogeneous. This heterogeneous nature presents challenges for a single model to accurately generate genomic sequences. In this paper, we analyze the properties of AR models and DMs in heterogeneous genomic sequence generation, pointing out crucial limitations in both methods: (i) AR models capture the underlying distribution of data by factorizing and learning the transition probability but fail to capture the global property of DNA sequences. (ii) DMs learn to recover the global distribution but tend to produce errors at the base pair level. To overcome the limitations of both approaches, we propose a post-training sampling method, termed Absorb & Escape (A&E) to perform compositional generation from AR models and DMs. This approach starts with samples generated by DMs and refines the sample quality using an AR model through the alternation of the Absorb and Escape steps. To assess the quality of generated sequences, we conduct extensive experiments on 15 species for conditional and unconditional DNA generation. The experiment results from motif distribution, diversity checks, and genome integration tests unequivocally show that A&E outperforms state-of-the-art AR models and DMs in genomic sequence generation.

==> sections/rebuttal.tex <==

\begin{table}[h!]
    \centering
       \small
        \caption{\textbf{Evaluation of transcription profile conditioned promoter sequence design.} \textsf{A\&E} achieves the smallest MSE with Language Model and DFM distilled being the AR and DM components.
    }
    \begin{tabular}{l c}
        \toprule
        \textbf{Method} & \textbf{MSE$\downarrow$} \\
        \midrule
        \textbf{Bit Diffusion (bit-encoding)*} & .0414 \\
        \textbf{Bit Diffusion (one-hot encoding)*} & .0395 \\
        \textbf{D3PM-uniform*} & .0375 \\
        \textbf{DDSM*} & .0334 \\
        \textbf{Language Model*} & .0333 \\
        \textbf{Linear FM*} & .0281 \\
        \textbf{Dirichlet FM (DFM)*} & .0269 \\
        \textbf{Dirichlet FM distilled (DFM distilled)*} & .0278 \\
        \midrule
        \textbf{ A\&E (Language Model+Dirichlet FM distilled)} & \textbf{.0262} \\
        \bottomrule
    \end{tabular}
    \label{tab:comparison}
    \vskip -0.2in
\end{table}

\paragraph{Landscape of EPD Dataset}
The construction process of EPD dataset are shown in \Cref{pic:epd-dataset} (a). The dataset, collected as of August 2023, involved downloading files through FTP and accessing fasta data via a graphical interface. Each sequence consists of promoeter and downstream protein encoding sequences, categorized as ‘promoter’ and ‘downstream’. Our compiled dataset consists of 30 million samples with various expression value and cell types. Then aggregated to 159,125 unique upstream-downstream sequences from 15 species.
\begin{figure*}[ht]
    \begin{center}
    \centerline{\includegraphics[width=\linewidth]{figures/ICML_dataset.pdf}}
    \caption{Generation Task with EPD-GenDNA. \textbf{(a) Dataset:} The EPD-GenDNA dataset includes 160K unique sequences from 15 species and 30 million samples with associated metadata.
\textbf{(b) Generative Modelling} Model $p_{\theta}(s)$ is trained to generate new DNA sequences.
\textbf{(c) Model Evaluation} }
        \label{pic:epd-dataset}
    \end{center}
    \vskip -0.2in
    % https://app.diagrams.net/#HZehui127%2Fdrawio%2Fmain%2FICML_dataset.drawio
\end{figure*}
\paragraph{Sensitivity Analysis}
We perform a \textit{sensitivity analysis} of A\&E algorithm over hyperparameter \( T_{\text{absorb}} \). As shown in \Cref{fig:Absorb-Escape-trade-off}, with a small \( T_{\text{absorb}} \), the sequences generated by A\&E are dominated by the diffusion model. As \( T_{\text{absorb}} \) increases, the AR helps to correct the errors made by the DM. Finally, when \( T_{\text{absorb}} \) is larger than 0.7, the correlation flattens and fluctuates. In conclusion, A\&E is robust under different values of \( T_{\text{absorb}} \), and it is best to use the validation dataset to choose the optimal value. However, a wide range of \( T_{\text{absorb}} \) can still be used with improved performance.

\begin{figure}[ht]
    \vskip 0.2in
    \begin{center}
    \centerline{\includegraphics[width=0.6\columnwidth]{figures/trade_off_init_only.pdf}}
        \caption{\textbf{Sensitivity of A\&E under various \( T_{\text{absorb}} \)}. For each value of \( T_{\text{absorb}} \), 3000 sequences are generated and compared with natural DNA. The correlation between the generated sequences and natural DNA increases initially as \( T_{\text{absorb}} \) increases, and then it flattens. An optimal \( T_{\text{absorb}} \) can be selected based on the validation set, or a default value of 0.85 can be used.}
        \label{fig:Absorb-Escape-trade-off}
    \end{center}
    \vskip -0.2in
\end{figure}



==> sections/related_work.tex <==
\section{Related Work}

Related work can be categorized into two groups: deep generative models for DNA generation, and evaluation methods for DNA generatoin. For the related work in generating from composed model, please refer to \Cref{app:related work}.

\paragraph{Deep Generative Models for Discrete Data}

\paragraph{DNA generation}

